Parameter Sensitivity of Deep-Feature based Evaluation Metrics for Audio Textures

Standard evaluation metrics such as the Inception score and Fr\'echet Audio Distance provide a general audio quality distance metric between the synthesized audio and reference clean audio. However, the sensitivity of these metrics to variations in the statistical parameters that define an audio texture is not well studied. In this work, we provide a systematic study of the sensitivity of some of the existing audio quality evaluation metrics to parameter variations in audio textures. Furthermore, we also study three more potentially parameter-sensitive metrics for audio texture synthesis, (a) a Gram matrix based distance, (b) an Accumulated Gram metric using a summarized version of the Gram matrices, and (c) a cochlear-model based statistical features metric. These metrics use deep features that summarize the statistics of any given audio texture, thus being inherently sensitive to variations in the statistical parameters that define an audio texture. We study and evaluate the sensitivity of existing standard metrics as well as Gram matrix and cochlear-model based metrics to control-parameter variations in audio textures across a wide range of texture and parameter types, and validate with subjective evaluation. We find that each of the metrics is sensitive to different sets of texture-parameter types. This is the first step towards investigating objective metrics for assessing parameter sensitivity in audio textures.

==> ParamSensing_ISMIR2022 (2)/SoundDataset.tex <==

\section{Synthetic Sound Data sets}
\label{appendix:synthetic}
Most of the sounds used in this paper come from the Syntex collection of datasets\footnote{https://syntex.sonicthings.org/}. Each dataset is generated by a different synthesis algorithm, and each file in a set is generated by sampling parameters of the algorithm. The dataset names are mnemonic and suggestive of the sound and types of parameters the algorithms expose (and not meant to make any claims about the ``realism" of sounds named). Here we describe how the various datasets in the collection are generated. The source code is also available at the syntex web site.

\subsection{DS\_BasicFM\_1.0}
A basic frequency modulation algorithm:
\[
  y[t]=sin(2\pi\, cf \,t + mI\, sin(2\pi \,mf \,t)))
\]
Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp (controls center frequency): $cf = 330*2^{cf\_exp}$; ranging in $[.2, .8]$, or fixed at $.5$.
\item mf (modulation frequency): ranging in $[0,20]$, or fixed at $10$.
\item mI (modulation index): ranging in $[5, 20]$, or fixed at $12.5$
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: FM-mf, FM-mi, and FM-cf, were prepared using this algorithm.
\subsection{DS\_Wind\_1.0}
Wind is constructed starting with a normally distributed white noise source followed by a 5th-order low-pass filter with a cutoff frequency of 400 Hz. This is followed by a band pass filter with time-varying center frequency (``cf") and gain, and a constant bandwidth value. 

The variation (cf and gain of the bandpass filter) is determined by a 1-dimensional simplex noise signal that is bounded (before scaling) in $[-1,1]$ and band-limited (we use the OpenSimplex\footnote{https://pypi.org/project/opensimplex/} python library). 

The simplex noise generator takes a frequency argument linearly proportional to the ``gustiness" parameter for the sound. A ``howliness" parameter controls the bandpass filter width parameter. A ``strength" parameter controls the average frequency around which the cf of the wind gusts fluctuate. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item strength: (controlling cf of bandpass filter): $cf=average\_cf*2^{.45*simplex\_signal}$, $average\_cf=180+440*strength$; $strength$ ranging in $[0,1]$, or fixed at $.5$.
\item gustiness: (controls frequency argument to simplex noise): $frequency=3*gustiness$; $gustiness$ ranging in $[0,1]$, or fixed at $.5$.
\item howliness (controlling bandwidth Q of the bandpass filter): $Q = .5+40*howliness$; $howliness$ ranging in $[0,1]$, or fixed at $.75$.
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: wind-gust, wind-howl, and wind-strength, were prepared using this algorithm.


\subsection{DS\_WindChimes\_1.0}
Five different ``chimes" ring at average rates that are a function of wind strength (wind also plays in the background for this sound). Each chime is constructed from 5 exponentially decaying sinusoidal signals with frequency, amplitude, and decay rates based on the empirical data reported in \cite{lukkari2004modal}. A ``chimeSize'' parameter for this sound scales all the chime frequencies.

A simplex noise signal is computed for each chime based on the wind ``strength" as described for DS\_Wind\_1.0 above. Zero-crossings in the simplex wave cause the corresponding chime to ring at an amplitude proportional to the derivative of the simplex signal at the zero crossing. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item strength: (see DS\_Wind\_1.0 above); $strength$ ranging in $[.2,.8]$, or fixed at $.5$.
\item chimeSize (controls scale\_factor for chime frequencies): $scale\_factor$ = $4*chimeSize$; $chimeSize$ ranging in $[.2,8]$, or fixed at $.5$.
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: windchimes-size, windchimes-strength, were prepared using this algorithm.


\subsection{DS\_Tapping1.2\_1.0}
This sound is based on the ``Tapping 1-2" on sound from \cite{mcdermott2011sound} paper on texture perception. The original sound consists of 10 regularly spaced pairs of taps over seven seconds with the second tap coming one quarter of the way through the repeating cycle period. DS\_Tapping1.2\_1.0 resynthesises this sound with parameters for the cycle period and for the phase in the cycle of the second tap. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item rate\_exp: $cycle\_rate = 2^{rate\_exp}$; $rate\_exp$ ranging in $[.5, 2]$, or fixed at $2$.
\item phase\_rel (phase of second tap in cycle): ranging in $[.2, .4]$, or fixed at $.3$
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: tapping-rate, and tapping-relphase, were prepared using this algorithm.


\subsection{DS\_Bees\_3.0}
Roughly imitative of a group of bees buzzing and moving around in a small space. Each bee buzz is created with an asymmetric triangle wave with an average center frequency in the vicinty of 200 Hz. The buzz source is followed by some formant-like filtering. Bees move toward and away from the listener based on a 1-dimensional simplex noise signal controlled by a frequency parameter for the simplex noise generator, and a maximum and minimum distance. This motion creates some variation in the buzzing frequency and amplitude due to the Doppler effect and amplitude roll-off with squared distance. These parameters are all fixed (the simplex frequency parameter is 2 Hz, the minimum and maximum distances are 2 and 10 meters.

There are two parameters systematically varied for the experiments in this paper. One is the center frequency of a Gaussian distribution from which each bee's average center frequency is drawn. 

Buzzes also have a  ``micro" variation in frequency following a 1-D simplex noise signal parameterized with a frequency argument of 14 Hz. The ``busybodyFreqFactor" controls the excursion of these micro variations by multiplying the [-1,1] simplex noise signal to get frequency variation in octaves. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp (exponent for the mean of a Gaussian distribution from which center frequencies of bee buzzes are drawn): $mean\_frequency = 440*2^{cf\_exp}$, the Gaussian has a fixed standard deviation of $.25$; $cf\_exp$ ranging in $[-2, 0]$,  or fixed at $1$.
\item busybodyFreqFactor (excursion in octaves): ranging in $[0, .5]$, or fixed at $.25$
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: bees-cf, and bees-busy, were prepared using this algorithm.

\subsection{DS\_Chirp\_1.0}
Chirps are frequency sweeps of a pitched tone with 3 harmonics (frequencies at [0, 1, and 2] times the fundamental). They have a center frequency (expressed in octaves relative to 400 Hz, see below) drawn from a Gaussian distribution, a duration, and move linearly in octaves. Chirps occur with an average number of events per second (eps), and can be spaced regularly (identically) in time, or irregularly according to a parameter (``irreg\_exp") (See Figure 
\ref{fig:irreg}).
\begin{figure}[h]
    \centering
    \subfigure[]{\includegraphics[width=0.6\textwidth]{images/irreg_0.0.png}} \vspace{-.5em}%
    \subfigure[]{\includegraphics[width=0.6\textwidth]{images/irreg_0.5.png}} \vspace{-.5em}%
    \subfigure[]{\includegraphics[width=0.6\textwidth]{images/irreg_1.0.png}}
    \caption{Histograms of events with a rate of 1/sec with 3 different irregularity parameters values, (a) 0.0, (b) 0.5, and (c), 1.0}
    \label{fig:irreg}
\end{figure}

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp: mean frequency of the Gaussian from which the center frequency of chirps is drawn $=440*2^{cf\_exp}$; $cf\_exp$ ranging in [0, 1], or fixed at $.5$.
\item irreg\_exp (standard deviation of Gaussian around regularly spaced events normalized by events per second (eps)): $sd=(.1*irreg\_exp*10^{irreg\_exp})/eps$; $irreg\_exp$ ranging in $[0, 1]$, or fixed at $0$ (see Figure \ref{fig:irreg}).
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: chirps-rate, chirps-cf, and chirps-irreg, were prepared using this algorithm.
\subsection{DS\_FBNoiseDelay\_1.0}
Uniformly distributed (``white") noise signal $x$ comb filtered using feed back delay:

\[
    y[n]=(1-\alpha)x[n]+\alpha y[n-K]
\]

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp (determines $K$): $K=sr/(220*2^{cf\_exp})$, $cf\_exp$ in [-1, 3], sr is sample rate. Resulting pitch in $[110, 880]$ Hz; $cf\_exp$ fixed at 0.
\item pitchedness (determines $\alpha$): $\alpha=1-1/2^{4*pitchedness}$, determines the bandwidth of the noise peaks at the harmonics of the nominal pitch frequency;  $pitchedness$ ranging in $[0,1)$ 
\end{itemize}
\textbf{Note}: The texture-param dataset of this paper: fbnoise-pitchedness, was prepared using this algorithm.

\subsection{DS\_Pops\_3.0}
Pops are generated by a brief noise burst (3 uniformly distributed random noise samples in [-1,1]) followed by a narrow bandpass filter with a center frequency drawn from a narrow Gaussian distribution. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf: mean frequency of a Gaussian from which the center frequency of the bandpass filter is drawn, and the standard deviation is 1 in units of musical semitones; $cf$ in $[540, 720]$ Hz, or fixed at $630$ Hz.
\item irreg\_exp (standard deviation of Gaussian around regularly spaced events normalized by events per second (eps)): $sd=(.1*irreg\_exp*10^{irreg\_exp})/eps$; $irreg\_exp$ ranging in $[.33, .66]$, or fixed at 0 (see Figure \ref{fig:irreg}).
\item rate\_exp:  $events per second =  2^{rate\_exp}$, $rate\_exp$ ranging in $[3, 4]$ or fixed at $4$.
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: pop-rate, pop-cf, and pop-irreg, were prepared using this algorithm.

\subsection{DS\_Applause\_w.0}
Individual claps are generated using the Pops model (above) but with noise bursts of 45 samples followed by band pass filters uniformly distributed in [800, 1400] Hz. Clapper sequences are generated with inter-clap intervals normally and narrowly distributed around .5 secs with slight periodic irregularity (Figure \ref{fig:irreg} to avoid unrealistic alignment between different clappers. Reverb\footnote{https://github.com/spotify/pedalboard} is used to create a basic room characteristic. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item numClappers\_exp: number of clappers = $2^{numClappers\_exp}$; $numClappers\_exp$ ranging  in $[1,3]$, or fixed: $2$.
\item rate\_exp :  rate (events per second) =  $2^{rate\_exp}$; $rate\_exp$  ranging: in $[1,2]$, or fixed: 2

\end{itemize}


\section{Recorded Sound Data sets}
\label{appendix:recorded}
We used three recorded datasets that have reasonably accurate labels for systematic parameter variation.

\subsection{NSynth}
The NSynth data set \cite{engel2017neural} contains over 300K musical notes from over 1K instruments systematically sampled and labeled over their respective ranges of chromatic pitch values (as well as other qualities). We used a subset consisting of one octave of 13 chromatic pitches for a brass instrument, with amplitude scaling at 10 different values. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item pitch: one octave of MIDI notes in [64, 76] which are musical notes from E4 (fundamental frequency 329.63 Hz) to E5 (659.26). Variations created with linear scalings of each note by 10 values in [.1, 1]
\end{itemize}
\textbf{Note}: The texture-param dataset of this paper: nsynth-pitch, refers to this dataset.


\subsection{Bucket filling with water}
This data set was recorded by filling a bucket with water poured from another bucket. The bucket was metal and had a capacity of 2.5 gallons. It was (repeatedly) filled at an approximately constant rate over a duration of 30 seconds. The transient sounds at the beginning and end of each sound was trimmed, and then sound was divided into 11 equally spaced time points used as the starting point of a 2-second excerpt labeled with one of 11 different ``fill levels" in [0,1].  Variations for different fill levels come from the multiple fillings. 
Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item fill level: ranging in $[0,1]$, variations taken from multiple recordings.
\end{itemize}
\textbf{Note}: The texture-param dataset of this paper: water-fill, refers to this dataset.

\subsection{Amen break}
The Amen Break is a loop of the first 2 bars of the famous and often-sampled drum break played by Gregory Coleman of the Winstons on the track, "Amen Brother." Variations in speed (without pitch change) were made using Audacity\footnote{https://www.audacityteam.org/} signal processing tools at intervals of one semitone.

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item tempo (relative to original): $original\_speed * 2^{n/12}$; $n$ ranging in $[-5,5]$ or fixed at $0$.
\item reverb : ranging in $[0,1]$ (dry to wet), or fixed at $.5$. 
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: drum-tempo and drum-rev, refer to this dataset.

\section{Gram-Matrix - details}
\label{appendix:AGM}
\subsection{Gram-Matrix Computation}
\label{appendix:gmcomputation}
The Gram-matrix for the $n^{th}$ CNN is computed as the time-averaged correlations between the feature maps from the filters.
Specifically, each element of the Gram-matrix of the $n^{th}$ CNN is defined as 
\begin{equation}
    G_{pq}^n = \sum_{m=1}^M f_{pm}^n\cdot f_{qm}^n
    = \vb{f}_p^n\cdot (\vb{f}_q^n)^T
\end{equation}
where, $M$ is the total number of time frames, $\vb{f}_p$ and $\vb{f}_q$ are the feature maps of dimension $1 \times M$ of the $p^{th}$ and the $q^{th}$ filters, where $p$ and $q$ range from 1 to the number of filters,$F$, i.e.~512. The resulting Gram-matrix, thus, has dimensions $512\times512$ at the output of each CNN, and the Gram-matrix of the $n^{th}$ CNN consists of dot products of the feature maps, written as,
\begin{gather}
    G = \begin{bmatrix}
\langle \vb{f}_1,\vb{f}_1\rangle&\langle \vb{f}_1,\vb{f}_2\rangle&..&\langle \vb{f}_1,\vb{f}_F\rangle\\
\langle \vb{f}_2,\vb{f}_1\rangle&\langle \vb{f}_2,\vb{f}_2\rangle&..&\langle \vb{f}_2,\vb{f}_F\rangle\\
...\\
\langle \vb{f}_F,\vb{f}_1\rangle&\langle \vb{f}_F,\vb{f}_2\rangle&..&\langle \vb{f}_F,\vb{f}_F\rangle
\label{eq:GM}
\end{bmatrix}
\end{gather}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{images/gm_metric.png}
%     \caption{Gram-Matrix param-sensing metric computation block diagram that consists of an ensemble of six 1 layer 1d-CNNs, with different kernel sizes, k. Each CNN has 512 filters, and the weights are randomly initialized. GM metric is computed from the gram matrices G.
% }
%     \label{fig:grammetric}
% \end{figure}

\subsection{Sparsity of Gram-Matrix}
\label{appendix:gmhistogram}
Figure \ref{fig:hist} shows the histogram of the values of the Gram matrices from the first ($k_1=2$) and the sixth ($k_6=128$) CNNs from a Frequency Modulation (FM) signal at a particular carrier frequency, modulation frequency, and modulation index and a water-filling sound at a particular fill level in a container. Although the range of values in these Gram-matrices are different (x-axis), it is evident from the histograms of the Gram-matrices of both these textures that they are sparse with most values of the matrix being close to zero. This suggests that non-zero values of the correlation between feature maps are sparsely located.

\begin{figure}
  \centering
  \begin{subfigure}[]{
    \includegraphics[width=0.5\columnwidth]{images/FM.png}}
  \end{subfigure}
  \begin{subfigure}[]{
    \includegraphics[width=0.5\columnwidth]{images/waterfill.png}}
  \end{subfigure}
  \caption{Histogram plots of the values of Gram-matrices from the first (k=2) and the sixth (k=128) CNNs. The top two plots are from a frequency modulation (FM) texture and the bottom two plots are from a water-filling texture.}
  \label{fig:hist}
\end{figure}


\subsection{Gram Vector Computation}
\label{appendix:gmvector}
We divide each row of the Gram matrix from equation \ref{eq:GM} into segments of length $s$, as shown in equation \ref{eq:GM2}, where in our experiments, we use $s=128$. 
\begin{gather}
    G = \begin{bmatrix}
\langle \vb{f}_1,\vb{f}_1\rangle&\langle \vb{f}_1,\vb{f}_2\rangle&..&\langle \vb{f}_1,\vb{f}_s\rangle&.......&\langle \vb{f}_1,\vb{f}_F\rangle\\
\langle \vb{f}_2,\vb{f}_1\rangle&\langle \vb{f}_2,\vb{f}_2\rangle&..&\langle \vb{f}_2,\vb{f}_s\rangle&.......&\langle \vb{f}_2,\vb{f}_F\rangle\\
...\\
\langle \vb{f}_F,\vb{f}_1\rangle&\langle \vb{f}_F,\vb{f}_2\rangle&..&\langle \vb{f}_F,\vb{f}_s\rangle&.......&\langle \vb{f}_F,\vb{f}_F\rangle
\end{bmatrix}
\label{eq:GM2}
\end{gather}

The Gram vector of dimension $1\times s$ is computed as a row aggregated average vector over all the Gram matrices of a given audio texture.
The first element of the Gram vector of the Gram-matrix from the $n^{th}$ CNN is computed as 
\begin{equation}
    g^n_1 = \frac{1}{4}\cdot\frac{1}{F}(\sum_{i=1}^F\langle \vb{f}_i,\vb{f}_1\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{s+1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{2s+1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{3s+1}\rangle)
\end{equation}

Similarly, the last element of this vector for the Gram-matrix from the ${n^{th}}$ CNN is computed as,
\begin{equation}
    g_s^n = \frac{1}{4}\cdot\frac{1}{F}(\sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{s-1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{2s-1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{3s-1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{4s-1}\rangle)
\end{equation}

Therefore, the overall gram vector $g$ of dimension $1\times s$ is the element-wise mean of these vectors over the $N$ Gram matrices of an audio texture corresponding to the CNNs, given as 
\begin{gather}
    g = \begin{bmatrix}
    \frac{1}{N}\sum_{n=1}^N g_1^n & \frac{1}{N}\sum_{n=1}^N g_2^n &...&\frac{1}{N}\sum_{n=1}^N g_s^n 
    \end{bmatrix}
\end{gather}

\section{Cochlear Param-Metric (CPM) - details}
\label{appendix:CPM}
The implementation uses a cochlear filterbank with 36 Gammatone filters, with Hilbert transform to compute the envelopes, and then compresses the envelopes with an exponential rate of 0.3 on each element in the matrix. The modulation filterbank with 20 filters is applied on each envelope, thus generating 36$\times$20 modulation bands. 

For each sound $x$, seven sets of statistics are computed, denote them by $S^i$ where $i=[1...7]$, 
\begin{itemize}[noitemsep,topsep=0pt]
    % \setlength\itemsep{-0.1em}
    \item Sub-band envelope power: average of the square sum, 36$\times$1.
    \item Sub-band envelope marginal statistics: mean, variance, skewness, kurtosis, 36$\times$4.
    \item Sub-band envelope variance: 36$\times$1.
    \item Sub-band envelope correlations: the correlation between each envelope, 36$\times$36.
    \item Modulation power: average of the square sum of each modulation bands, 36$\times$20.
    \item Modulation variance: 36$\times$20.
    \item Modulation correlation: the correlation between the same modulation bands for every 2-step nearest envelopes, in total (36$\times$5-6)$\times$20 = 3,480. 
\end{itemize}
The algorithm, thus, generates 6,432 statistical parameters.

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{images/mcdermott-diagram.png}
    \caption{CPM from the statistics derived from \cite{mcdermott2011sound}. Red icons denote the statistical measurements: P: power, M: marginal statistics, V: variance, C: correlations between subbands as described above.}
    \label{fig:CPM}
\end{figure}

% \pagebreak
\section{Comparison plots for objective metrics with human perceptual measures}
\label{appendix:HUMANPLOTS}
The trends of subjective responses and objective metrics can be observed for the three sets of audio textures in Figures \ref{fig:appendix-comparison-pitched} (pitched), \ref{fig:appendix-comparison-rhythmic} (rhythmic), and \ref{fig:appendix-comparison-others} (others). 
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/pitched.png}
    \caption{Comparison plots for pitched sounds}
    \label{fig:appendix-comparison-pitched}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/rhythmic.png}
    \caption{Comparison plots for rhythmic sounds}
    \label{fig:appendix-comparison-rhythmic}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/others.png}
    \caption{Comparison plots for other sounds}
    \label{fig:appendix-comparison-others}
\end{figure*}

\section{Human Listening Test Plots}
\label{appendix:listeningtestplots}
The rank-order responses obtained from the human listening tests are plotted in Figure \ref{fig:appendix-human-test-ranks-all}.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/human-test-ranks-all.png}
    \caption{Plots showing rank orders captured from human listening tests (y-axis) w.r.t control parameter (x-axis) used to generate the audio samples. Error bars show the standard deviation of the ranks collected at each control parameter.}
    \label{fig:appendix-human-test-ranks-all}
\end{figure*}



==> SoundDataset.tex <==

\section{Synthetic Sound Data sets}
\label{appendix:synthetic}
Most of the sounds used in this paper come from the Syntex collection of datasets\footnote{https://syntex.sonicthings.org/}. Each dataset is generated by a different synthesis algorithm, and each file in a set is generated by sampling parameters of the algorithm. The dataset names are mnemonic and suggestive of the sound and types of parameters the algorithms expose (and not meant to make any claims about the ``realism" of sounds named). Here we describe how the various datasets in the collection are generated. The source code is also available at the syntex web site.

\subsection{DS\_BasicFM\_1.0}
A basic frequency modulation algorithm:
\[
  y[t]=sin(2\pi\, cf \,t + mI\, sin(2\pi \,mf \,t)))
\]
Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp (controls center frequency): $cf = 330*2^{cf\_exp}$; ranging in $[.2, .8]$, or fixed at $.5$.
\item mf (modulation frequency): ranging in $[0,20]$, or fixed at $10$.
\item mI (modulation index): ranging in $[5, 20]$, or fixed at $12.5$
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: FM-mf, FM-mi, and FM-cf, were prepared using this algorithm.
\subsection{DS\_Wind\_1.0}
Wind is constructed starting with a normally distributed white noise source followed by a 5th-order low-pass filter with a cutoff frequency of 400 Hz. This is followed by a band pass filter with time-varying center frequency (``cf") and gain, and a constant bandwidth value. 

The variation (cf and gain of the bandpass filter) is determined by a 1-dimensional simplex noise signal that is bounded (before scaling) in $[-1,1]$ and band-limited (we use the OpenSimplex\footnote{https://pypi.org/project/opensimplex/} python library). 

The simplex noise generator takes a frequency argument linearly proportional to the ``gustiness" parameter for the sound. A ``howliness" parameter controls the bandpass filter width parameter. A ``strength" parameter controls the average frequency around which the cf of the wind gusts fluctuate. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item strength: (controlling cf of bandpass filter): $cf=average\_cf*2^{.45*simplex\_signal}$, $average\_cf=180+440*strength$; $strength$ ranging in $[0,1]$, or fixed at $.5$.
\item gustiness: (controls frequency argument to simplex noise): $frequency=3*gustiness$; $gustiness$ ranging in $[0,1]$, or fixed at $.5$.
\item howliness (controlling bandwidth Q of the bandpass filter): $Q = .5+40*howliness$; $howliness$ ranging in $[0,1]$, or fixed at $.75$.
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: wind-gust, wind-howl, and wind-strength, were prepared using this algorithm.


\subsection{DS\_WindChimes\_1.0}
Five different ``chimes" ring at average rates that are a function of wind strength (wind also plays in the background for this sound). Each chime is constructed from 5 exponentially decaying sinusoidal signals with frequency, amplitude, and decay rates based on the empirical data reported in \cite{lukkari2004modal}. A ``chimeSize'' parameter for this sound scales all the chime frequencies.

A simplex noise signal is computed for each chime based on the wind ``strength" as described for DS\_Wind\_1.0 above. Zero-crossings in the simplex wave cause the corresponding chime to ring at an amplitude proportional to the derivative of the simplex signal at the zero crossing. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item strength: (see DS\_Wind\_1.0 above); $strength$ ranging in $[.2,.8]$, or fixed at $.5$.
\item chimeSize (controls scale\_factor for chime frequencies): $scale\_factor$ = $4*chimeSize$; $chimeSize$ ranging in $[.2,8]$, or fixed at $.5$.
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: windchimes-size, windchimes-strength, were prepared using this algorithm.


\subsection{DS\_Tapping1.2\_1.0}
This sound is based on the ``Tapping 1-2" on sound from \cite{mcdermott2011sound} paper on texture perception. The original sound consists of 10 regularly spaced pairs of taps over seven seconds with the second tap coming one quarter of the way through the repeating cycle period. DS\_Tapping1.2\_1.0 resynthesises this sound with parameters for the cycle period and for the phase in the cycle of the second tap. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item rate\_exp: $cycle\_rate = 2^{rate\_exp}$; $rate\_exp$ ranging in $[.5, 2]$, or fixed at $2$.
\item phase\_rel (phase of second tap in cycle): ranging in $[.2, .4]$, or fixed at $.3$
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: tapping-rate, and tapping-relphase, were prepared using this algorithm.


\subsection{DS\_Bees\_3.0}
Roughly imitative of a group of bees buzzing and moving around in a small space. Each bee buzz is created with an asymmetric triangle wave with an average center frequency in the vicinty of 200 Hz. The buzz source is followed by some formant-like filtering. Bees move toward and away from the listener based on a 1-dimensional simplex noise signal controlled by a frequency parameter for the simplex noise generator, and a maximum and minimum distance. This motion creates some variation in the buzzing frequency and amplitude due to the Doppler effect and amplitude roll-off with squared distance. These parameters are all fixed (the simplex frequency parameter is 2 Hz, the minimum and maximum distances are 2 and 10 meters.

There are two parameters systematically varied for the experiments in this paper. One is the center frequency of a Gaussian distribution from which each bee's average center frequency is drawn. 

Buzzes also have a  ``micro" variation in frequency following a 1-D simplex noise signal parameterized with a frequency argument of 14 Hz. The ``busybodyFreqFactor" controls the excursion of these micro variations by multiplying the [-1,1] simplex noise signal to get frequency variation in octaves. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp (exponent for the mean of a Gaussian distribution from which center frequencies of bee buzzes are drawn): $mean\_frequency = 440*2^{cf\_exp}$, the Gaussian has a fixed standard deviation of $.25$; $cf\_exp$ ranging in $[-2, 0]$,  or fixed at $1$.
\item busybodyFreqFactor (excursion in octaves): ranging in $[0, .5]$, or fixed at $.25$
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: bees-cf, and bees-busy, were prepared using this algorithm.

\subsection{DS\_Chirp\_1.0}
Chirps are frequency sweeps of a pitched tone with 3 harmonics (frequencies at [0, 1, and 2] times the fundamental). They have a center frequency (expressed in octaves relative to 400 Hz, see below) drawn from a Gaussian distribution, a duration, and move linearly in octaves. Chirps occur with an average number of events per second (eps), and can be spaced regularly (identically) in time, or irregularly according to a parameter (``irreg\_exp") (See Figure 
\ref{fig:irreg}).
\begin{figure}[h]
    \centering
    \subfigure[]{\includegraphics[width=0.6\textwidth]{images/irreg_0.0.png}} \vspace{-.5em}%
    \subfigure[]{\includegraphics[width=0.6\textwidth]{images/irreg_0.5.png}} \vspace{-.5em}%
    \subfigure[]{\includegraphics[width=0.6\textwidth]{images/irreg_1.0.png}}
    \caption{Histograms of events with a rate of 1/sec with 3 different irregularity parameters values, (a) 0.0, (b) 0.5, and (c), 1.0}
    \label{fig:irreg}
\end{figure}

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp: mean frequency of the Gaussian from which the center frequency of chirps is drawn $=440*2^{cf\_exp}$; $cf\_exp$ ranging in [0, 1], or fixed at $.5$.
\item irreg\_exp (standard deviation of Gaussian around regularly spaced events normalized by events per second (eps)): $sd=(.1*irreg\_exp*10^{irreg\_exp})/eps$; $irreg\_exp$ ranging in $[0, 1]$, or fixed at $0$ (see Figure \ref{fig:irreg}).
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: chirps-rate, chirps-cf, and chirps-irreg, were prepared using this algorithm.
\subsection{DS\_FBNoiseDelay\_1.0}
Uniformly distributed (``white") noise signal $x$ comb filtered using feed back delay:

\[
    y[n]=(1-\alpha)x[n]+\alpha y[n-K]
\]

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf\_exp (determines $K$): $K=sr/(220*2^{cf\_exp})$, $cf\_exp$ in [-1, 3], sr is sample rate. Resulting pitch in $[110, 880]$ Hz; $cf\_exp$ fixed at 0.
\item pitchedness (determines $\alpha$): $\alpha=1-1/2^{4*pitchedness}$, determines the bandwidth of the noise peaks at the harmonics of the nominal pitch frequency;  $pitchedness$ ranging in $[0,1)$ 
\end{itemize}
\textbf{Note}: The texture-param dataset of this paper: fbnoise-pitchedness, was prepared using this algorithm.

\subsection{DS\_Pops\_3.0}
Pops are generated by a brief noise burst (3 uniformly distributed random noise samples in [-1,1]) followed by a narrow bandpass filter with a center frequency drawn from a narrow Gaussian distribution. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item cf: mean frequency of a Gaussian from which the center frequency of the bandpass filter is drawn, and the standard deviation is 1 in units of musical semitones; $cf$ in $[540, 720]$ Hz, or fixed at $630$ Hz.
\item irreg\_exp (standard deviation of Gaussian around regularly spaced events normalized by events per second (eps)): $sd=(.1*irreg\_exp*10^{irreg\_exp})/eps$; $irreg\_exp$ ranging in $[.33, .66]$, or fixed at 0 (see Figure \ref{fig:irreg}).
\item rate\_exp:  $events per second =  2^{rate\_exp}$, $rate\_exp$ ranging in $[3, 4]$ or fixed at $4$.
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: pop-rate, pop-cf, and pop-irreg, were prepared using this algorithm.

\subsection{DS\_Applause\_w.0}
Individual claps are generated using the Pops model (above) but with noise bursts of 45 samples followed by band pass filters uniformly distributed in [800, 1400] Hz. Clapper sequences are generated with inter-clap intervals normally and narrowly distributed around .5 secs with slight periodic irregularity (Figure \ref{fig:irreg} to avoid unrealistic alignment between different clappers. Reverb\footnote{https://github.com/spotify/pedalboard} is used to create a basic room characteristic. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item numClappers\_exp: number of clappers = $2^{numClappers\_exp}$; $numClappers\_exp$ ranging  in $[1,3]$, or fixed: $2$.
\item rate\_exp :  rate (events per second) =  $2^{rate\_exp}$; $rate\_exp$  ranging: in $[1,2]$, or fixed: 2

\end{itemize}


\section{Recorded Sound Data sets}
\label{appendix:recorded}
We used three recorded datasets that have reasonably accurate labels for systematic parameter variation.

\subsection{NSynth}
The NSynth data set \cite{engel2017neural} contains over 300K musical notes from over 1K instruments systematically sampled and labeled over their respective ranges of chromatic pitch values (as well as other qualities). We used a subset consisting of one octave of 13 chromatic pitches for a brass instrument, with amplitude scaling at 10 different values. 

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item pitch: one octave of MIDI notes in [64, 76] which are musical notes from E4 (fundamental frequency 329.63 Hz) to E5 (659.26). Variations created with linear scalings of each note by 10 values in [.1, 1]
\end{itemize}
\textbf{Note}: The texture-param dataset of this paper: nsynth-pitch, refers to this dataset.


\subsection{Bucket filling with water}
This data set was recorded by filling a bucket with water poured from another bucket. The bucket was metal and had a capacity of 2.5 gallons. It was (repeatedly) filled at an approximately constant rate over a duration of 30 seconds. The transient sounds at the beginning and end of each sound was trimmed, and then sound was divided into 11 equally spaced time points used as the starting point of a 2-second excerpt labeled with one of 11 different ``fill levels" in [0,1].  Variations for different fill levels come from the multiple fillings. 
Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item fill level: ranging in $[0,1]$, variations taken from multiple recordings.
\end{itemize}
\textbf{Note}: The texture-param dataset of this paper: water-fill, refers to this dataset.

\subsection{Amen break}
The Amen Break is a loop of the first 2 bars of the famous and often-sampled drum break played by Gregory Coleman of the Winstons on the track, "Amen Brother." Variations in speed (without pitch change) were made using Audacity\footnote{https://www.audacityteam.org/} signal processing tools at intervals of one semitone.

Parameters:
\begin{itemize}[noitemsep,nolistsep]
\item tempo (relative to original): $original\_speed * 2^{n/12}$; $n$ ranging in $[-5,5]$ or fixed at $0$.
\item reverb : ranging in $[0,1]$ (dry to wet), or fixed at $.5$. 
\end{itemize}
\textbf{Note}: The texture-param datasets of this paper: drum-tempo and drum-rev, refer to this dataset.

\section{Gram-Matrix - details}
\label{appendix:AGM}
\subsection{Gram-Matrix Computation}
\label{appendix:gmcomputation}
The Gram-matrix for the $n^{th}$ CNN is computed as the time-averaged correlations between the feature maps from the filters.
Specifically, each element of the Gram-matrix of the $n^{th}$ CNN is defined as 
\begin{equation}
    G_{pq}^n = \sum_{m=1}^M f_{pm}^n\cdot f_{qm}^n
    = \vb{f}_p^n\cdot (\vb{f}_q^n)^T
\end{equation}
where, $M$ is the total number of time frames, $\vb{f}_p$ and $\vb{f}_q$ are the feature maps of dimension $1 \times M$ of the $p^{th}$ and the $q^{th}$ filters, where $p$ and $q$ range from 1 to the number of filters,$F$, i.e.~512. The resulting Gram-matrix, thus, has dimensions $512\times512$ at the output of each CNN, and the Gram-matrix of the $n^{th}$ CNN consists of dot products of the feature maps, written as,
\begin{gather}
    G = \begin{bmatrix}
\langle \vb{f}_1,\vb{f}_1\rangle&\langle \vb{f}_1,\vb{f}_2\rangle&..&\langle \vb{f}_1,\vb{f}_F\rangle\\
\langle \vb{f}_2,\vb{f}_1\rangle&\langle \vb{f}_2,\vb{f}_2\rangle&..&\langle \vb{f}_2,\vb{f}_F\rangle\\
...\\
\langle \vb{f}_F,\vb{f}_1\rangle&\langle \vb{f}_F,\vb{f}_2\rangle&..&\langle \vb{f}_F,\vb{f}_F\rangle
\label{eq:GM}
\end{bmatrix}
\end{gather}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{images/gm_metric.png}
%     \caption{Gram-Matrix param-sensing metric computation block diagram that consists of an ensemble of six 1 layer 1d-CNNs, with different kernel sizes, k. Each CNN has 512 filters, and the weights are randomly initialized. GM metric is computed from the gram matrices G.
% }
%     \label{fig:grammetric}
% \end{figure}

\subsection{Sparsity of Gram-Matrix}
\label{appendix:gmhistogram}
Figure \ref{fig:hist} shows the histogram of the values of the Gram matrices from the first ($k_1=2$) and the sixth ($k_6=128$) CNNs from a Frequency Modulation (FM) signal at a particular carrier frequency, modulation frequency, and modulation index and a water-filling sound at a particular fill level in a container. Although the range of values in these Gram-matrices are different (x-axis), it is evident from the histograms of the Gram-matrices of both these textures that they are sparse with most values of the matrix being close to zero. This suggests that non-zero values of the correlation between feature maps are sparsely located.

\begin{figure}
  \centering
  \begin{subfigure}[]{
    \includegraphics[width=0.5\columnwidth]{images/FM.png}}
  \end{subfigure}
  \begin{subfigure}[]{
    \includegraphics[width=0.5\columnwidth]{images/waterfill.png}}
  \end{subfigure}
  \caption{Histogram plots of the values of Gram-matrices from the first (k=2) and the sixth (k=128) CNNs. The top two plots are from a frequency modulation (FM) texture and the bottom two plots are from a water-filling texture.}
  \label{fig:hist}
\end{figure}


\subsection{Gram Vector Computation}
\label{appendix:gmvector}
We divide each row of the Gram matrix from equation \ref{eq:GM} into segments of length $s$, as shown in equation \ref{eq:GM2}, where in our experiments, we use $s=128$. 
\begin{gather}
    G = \begin{bmatrix}
\langle \vb{f}_1,\vb{f}_1\rangle&\langle \vb{f}_1,\vb{f}_2\rangle&..&\langle \vb{f}_1,\vb{f}_s\rangle&.......&\langle \vb{f}_1,\vb{f}_F\rangle\\
\langle \vb{f}_2,\vb{f}_1\rangle&\langle \vb{f}_2,\vb{f}_2\rangle&..&\langle \vb{f}_2,\vb{f}_s\rangle&.......&\langle \vb{f}_2,\vb{f}_F\rangle\\
...\\
\langle \vb{f}_F,\vb{f}_1\rangle&\langle \vb{f}_F,\vb{f}_2\rangle&..&\langle \vb{f}_F,\vb{f}_s\rangle&.......&\langle \vb{f}_F,\vb{f}_F\rangle
\end{bmatrix}
\label{eq:GM2}
\end{gather}

The Gram vector of dimension $1\times s$ is computed as a row aggregated average vector over all the Gram matrices of a given audio texture.
The first element of the Gram vector of the Gram-matrix from the $n^{th}$ CNN is computed as 
\begin{equation}
    g^n_1 = \frac{1}{4}\cdot\frac{1}{F}(\sum_{i=1}^F\langle \vb{f}_i,\vb{f}_1\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{s+1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{2s+1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{3s+1}\rangle)
\end{equation}

Similarly, the last element of this vector for the Gram-matrix from the ${n^{th}}$ CNN is computed as,
\begin{equation}
    g_s^n = \frac{1}{4}\cdot\frac{1}{F}(\sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{s-1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{2s-1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{3s-1}\rangle + \sum_{i=1}^F\langle \vb{f}_i,\vb{f}_{4s-1}\rangle)
\end{equation}

Therefore, the overall gram vector $g$ of dimension $1\times s$ is the element-wise mean of these vectors over the $N$ Gram matrices of an audio texture corresponding to the CNNs, given as 
\begin{gather}
    g = \begin{bmatrix}
    \frac{1}{N}\sum_{n=1}^N g_1^n & \frac{1}{N}\sum_{n=1}^N g_2^n &...&\frac{1}{N}\sum_{n=1}^N g_s^n 
    \end{bmatrix}
\end{gather}

\section{Cochlear Param-Metric (CPM) - details}
\label{appendix:CPM}
The implementation uses a cochlear filterbank with 36 Gammatone filters, with Hilbert transform to compute the envelopes, and then compresses the envelopes with an exponential rate of 0.3 on each element in the matrix. The modulation filterbank with 20 filters is applied on each envelope, thus generating 36$\times$20 modulation bands. 

For each sound $x$, seven sets of statistics are computed, denote them by $S^i$ where $i=[1...7]$, 
\begin{itemize}[noitemsep,topsep=0pt]
    % \setlength\itemsep{-0.1em}
    \item Sub-band envelope power: average of the square sum, 36$\times$1.
    \item Sub-band envelope marginal statistics: mean, variance, skewness, kurtosis, 36$\times$4.
    \item Sub-band envelope variance: 36$\times$1.
    \item Sub-band envelope correlations: the correlation between each envelope, 36$\times$36.
    \item Modulation power: average of the square sum of each modulation bands, 36$\times$20.
    \item Modulation variance: 36$\times$20.
    \item Modulation correlation: the correlation between the same modulation bands for every 2-step nearest envelopes, in total (36$\times$5-6)$\times$20 = 3,480. 
\end{itemize}
The algorithm, thus, generates 6,432 statistical parameters.

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{images/mcdermott-diagram.png}
    \caption{CPM from the statistics derived from \cite{mcdermott2011sound}. Red icons denote the statistical measurements: P: power, M: marginal statistics, V: variance, C: correlations between subbands as described above.}
    \label{fig:CPM}
\end{figure}

% \pagebreak
\section{Comparison plots for objective metrics with human perceptual measures}
\label{appendix:HUMANPLOTS}
The trends of subjective responses and objective metrics can be observed for the three sets of audio textures in Figures \ref{fig:appendix-comparison-pitched} (pitched), \ref{fig:appendix-comparison-rhythmic} (rhythmic), and \ref{fig:appendix-comparison-others} (others). 
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/pitched.png}
    \caption{Comparison plots for pitched sounds}
    \label{fig:appendix-comparison-pitched}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/rhythmic.png}
    \caption{Comparison plots for rhythmic sounds}
    \label{fig:appendix-comparison-rhythmic}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/others.png}
    \caption{Comparison plots for other sounds}
    \label{fig:appendix-comparison-others}
\end{figure*}

\section{Human Listening Test Plots}
\label{appendix:listeningtestplots}
The rank-order responses obtained from the human listening tests are plotted in Figure \ref{fig:appendix-human-test-ranks-all}.
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/human-test-ranks-all.png}
    \caption{Plots showing rank orders captured from human listening tests (y-axis) w.r.t control parameter (x-axis) used to generate the audio samples. Error bars show the standard deviation of the ranks collected at each control parameter.}
    \label{fig:appendix-human-test-ranks-all}
\end{figure*}


